CAS-GAN for Contrast-free Angiography Synthesis

Iodinated contrast agents are widely utilized in numerous interventional procedures, yet posing substantial health risks to patients. This paper presents CAS-GAN, a novel GAN framework that serves as a "virtual contrast agent" to synthesize X-ray angiographies via disentanglement representation learning and vessel semantic guidance, thereby reducing the reliance on iodinated contrast agents during interventional procedures. Specifically, our approach disentangles X-ray angiographies into background and vessel components, leveraging medical prior knowledge. A specialized predictor then learns to map the interrelationships between these components. Additionally, a vessel semantic-guided generator and a corresponding loss function are introduced to enhance the visual fidelity of generated images. Experimental results on the XCAD dataset demonstrate the state-of-the-art performance of our CAS-GAN, achieving a FID of 5.87 and a MMD of 0.016. These promising results highlight CAS-GAN's potential for clinical applications.

==> Ablation_Loss.tex <==
\begin{table}[htbp]
\caption{
Effect of several loss functions on the XCAD dataset. FID is reported in this table.
}
\label{table:ablation_loss}
\centering
\renewcommand\arraystretch{1.2}
\renewcommand\arraystretch{1.2}
\begin{tabular}{cccll}
\toprule
\multicolumn{3}{c}{Loss functions} & \multirow{2}{*}{FID $\downarrow$} & \multirow{2}{*}{$\Delta$} \\ \cmidrule{1-3}
$\mathcal{L}_{\rm Cycle}^{\rm Lat}$ & $\mathcal{L}_{\rm Reconst}$ & $\mathcal{L}_{\rm Sem}$ & & \\ \midrule
 & & & $6.20$ & ${\color{blue}+0.26}$ \\
 & & \checkmark & & \\
 & \checkmark & & & \\
 & \checkmark & \checkmark & & \\
\checkmark & & & & \\
\checkmark & & \checkmark & & \\
\checkmark & \checkmark & & & \\
\checkmark & \checkmark & \checkmark & $5.94$ & $-$ \\ \bottomrule
\end{tabular}
\end{table}

==> ref_simple.tex <==
@article{roth2020global,
  title={The global burden of cardiovascular diseases and risks: A compass for global action},
  author={Roth, Gregory A and Mensah, George A and Fuster, Valentin},
  journal={JACC},
  volume={76},
  number={25},
  pages={2980--2981},
  year={2020}
}


@inproceedings{zhu2017unpaired,
  title={Unpaired image-to-image translation using cycle-consistent adversarial networks},
  author={Zhu, Jun-Yan and Park, Taesung and Isola, Phillip and Efros, Alexei A},
  booktitle={Proc. ICCV},
  pages={2223--2232},
  year={2017}
}


@inproceedings{park2020contrastive,
  title={Contrastive learning for unpaired image-to-image translation},
  author={Park, Taesung and Efros, Alexei A and Zhang, Richard and Zhu, Jun-Yan},
  booktitle={Proc. ECCV},
  pages={319--345},
  year={2020},
  organization={Springer}
}


@article{dar2019image,
  title={Image synthesis in multi-contrast {MRI} with conditional generative adversarial networks},
  author={Dar, Salman UH and Yurt, Mahmut and Karacan, Levent and Erdem, Aykut and Erdem, Erkut and Cukur, Tolga},
  journal={TMI},
  volume={38},
  number={10},
  pages={2375--2388},
  year={2019}
}


@article{nie2018medical,
  title={Medical image synthesis with deep convolutional adversarial networks},
  author={Nie, Dong and others},
  journal={TBME},
  volume={65},
  number={12},
  pages={2720--2730},
  year={2018}
}


@inproceedings{ma2021self,
  title={Self-supervised vessel segmentation via adversarial learning},
  author={Ma, Yuxin and others},
  booktitle={Proc. ICCV},
  pages={7536--7545},
  year={2021}
}


@inproceedings{zhang2019self,
  title={Self-attention generative adversarial networks},
  author={Zhang, Han and Goodfellow, Ian and Metaxas, Dimitris and Odena, Augustus},
  booktitle={Proc. ICML},
  pages={7354--7363},
  year={2019}
}


@article{tang2021attentiongan,
  title={{AttentionGAN}: Unpaired image-to-image translation using attention-guided generative adversarial networks},
  author={Tang, Hao and Liu, Hong and Xu, Dan and Torr, Philip HS and Sebe, Nicu},
  journal={TNNLS},
  volume={34},
  number={4},
  pages={1972--1987},
  year={2021}
}


@inproceedings{wu2024stegogan,
  title={{StegoGAN}: Leveraging Steganography for Non-Bijective Image-to-Image Translation},
  author={Wu, Sidi and others},
  booktitle={Proc. CVPR},
  pages={7922--7931},
  year={2024}
}


@inproceedings{hu2022qs,
  title={{QS-Attn}: Query-selected attention for contrastive learning in {I2I} translation},
  author={Hu, Xueqi and Zhou, Xinyue and Huang, Qiusheng and Shi, Zhengyi and Sun, Li and Li, Qingli},
  booktitle={Proc. CVPR},
  pages={18291--18300},
  year={2022}
}


@inproceedings{goodfellow2014generative,
  title={Generative adversarial nets},
  author={Goodfellow, Ian and others},
  booktitle={Proc. NeurIPS},
  volume={27},
  year={2014}
}


@article{guo2023medgan,
  title={{MedGAN}: An adaptive {GAN} approach for medical image generation},
  author={Guo, Kehua and others},
  journal={Computers in Biology and Medicine},
  volume={163},
  pages={107119},
  year={2023}
}


@article{yi2019generative,
  title={Generative adversarial network in medical imaging: A review},
  author={Yi, Xin and Walia, Ekta and Babyn, Paul},
  journal={Medical Image Analysis},
  volume={58},
  pages={101552},
  year={2019}
}

@article{kodali2017convergence,
  title={On convergence and stability of {GANs}},
  author={Kodali, Naveen and Abernethy, Jacob and Hays, James and Kira, Zsolt},
  journal={arXiv preprint arXiv:1705.07215},
  year={2017}
}

@inproceedings{tran2018dist,
  title={{Dist-GAN}: An improved {GAN} using distance constraints},
  author={Tran, Ngoc-Trung and Bui, Tuan-Anh and Cheung, Ngai-Man},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={370--385},
  year={2018}
}


@inproceedings{bang2021mggan,
  title={{MGGAN}: Solving mode collapse using manifold-guided training},
  author={Bang, Duhyeon and Shim, Hyunjung},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
  pages={2347--2356},
  year={2021}
}


@inproceedings{arjovsky2017wasserstein,
  title={Wasserstein generative adversarial networks},
  author={Arjovsky, Martin and Chintala, Soumith and Bottou, L{\'e}on},
  booktitle={Proceedings of the International Conference on Machine Learning (ICML)},
  pages={214--223},
  year={2017}
}


@inproceedings{paszke2019pytorch,
  title={{PyTorch}: An imperative style, high-performance deep learning library},
  author={Paszke, Adam and others},
  booktitle={Proceedings of the Advances in Neural Information Processing Systems (NeurIPS)},
  volume={32},
  year={2019}
}


@inproceedings{kingma2014adam,
  title={Adam: A method for stochastic optimization},
  author={Kingma, Diederik P and Ba, Jimmy},
  booktitle={Proceedings of the International Conference on Learning Representations (ICLR)},
  year={2014}
}


@article{moreno2020hybrid,
  title={The hybrid coronary approach for optimal revascularization: {JACC} review topic of the week},
  author={Moreno, Pedro R and Stone, Gregg W and Gonzalez-Lengua, Carlos A and Puskas, John D},
  journal={Journal of the American College of Cardiology},
  volume={76},
  number={3},
  pages={321--333},
  year={2020}
}


@inproceedings{heusel2017gans,
  title={{GANs} trained by a two time-scale update rule converge to a local nash equilibrium},
  author={Heusel, Martin and Ramsauer, Hubert and Unterthiner, Thomas and Nessler, Bernhard and Hochreiter, Sepp},
  booktitle={Proceedings of the Advances in Neural Information Processing Systems (NeurIPS)},
  volume={30},
  year={2017}
}


@inproceedings{huang2018multimodal,
  title={Multimodal unsupervised image-to-image translation},
  author={Huang, Xun and Liu, Ming-Yu and Belongie, Serge and Kautz, Jan},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={172--189},
  year={2018}
}


@article{mittal2012making,
  title={Making a “completely blind” image quality analyzer},
  author={Mittal, Anish and Soundararajan, Rajiv and Bovik, Alan C},
  journal={IEEE Signal Processing Letters},
  volume={20},
  number={3},
  pages={209--212},
  year={2012}
}


@inproceedings{salimans2016improved,
  title={Improved techniques for training {GANs}},
  author={Salimans, Tim and Goodfellow, Ian and Zaremba, Wojciech and Cheung, Vicki and Radford, Alec and Chen, Xi},
  booktitle={Proceedings of the Advances in Neural Information Processing Systems (NeurIPS)},
  volume={29},
  year={2016}
}


@inproceedings{mao2017least,
  title={Least squares generative adversarial networks},
  author={Mao, Xudong and Li, Qing and Xie, Haoran and Lau, Raymond YK and Wang, Zhen and Paul Smolley, Stephen},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision (ICCV)},
  pages={2794--2802},
  year={2017}
}


@inproceedings{park2023content,
  title={Content-aware local gan for photo-realistic super-resolution},
  author={Park, JoonKyu and Son, Sanghyun and Lee, Kyoung Mu},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
  pages={10585--10594},
  year={2023}
}


@article{tran2021data,
  title={On data augmentation for {GAN} training},
  author={Tran, Ngoc-Trung and Tran, Viet-Hung and Nguyen, Ngoc-Bao and Nguyen, Trung-Kien and Cheung, Ngai-Man},
  journal={IEEE Transactions on Image Processing},
  volume={30},
  pages={1882--1897},
  year={2021}
}


@article{pang2021image,
  title={Image-to-image translation: Methods and applications},
  author={Pang, Yingxue and Lin, Jianxin and Qin, Tao and Chen, Zhibo},
  journal={IEEE Transactions on Multimedia},
  volume={24},
  pages={3859--3881},
  year={2021}
}


@inproceedings{choi2020stargan,
  title={{StarGAN} v2: Diverse image synthesis for multiple domains},
  author={Choi, Yunjey and Uh, Youngjung and Yoo, Jaejun and Ha, Jung-Woo},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={8188--8197},
  year={2020}
}


@inproceedings{richardson2021encoding,
  title={Encoding in style: A {StyleGAN} encoder for image-to-image translation},
  author={Richardson, Elad and others},
  booktitle={Proceedings of the IEEE/CVF Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={2287--2296},
  year={2021}
}

@inproceedings{armanious2019unsupervised,
  title={Unsupervised medical image translation using cycle-{MedGAN}},
  author={Armanious, Karim and Jiang, Chenming and Abdulatif, Sherif and K{\"u}stner, Thomas and Gatidis, Sergios and Yang, Bin},
  booktitle={Proceedings of the 2019 27th European signal processing conference (EUSIPCO)},
  year={2019}
}


@article{martin2023unsupervised,
  title={Unsupervised synthesis of realistic coronary artery {X-ray} angiogram},
  author={Martin, R{\'e}mi and Segars, Paul and Samei, Ehsan and Mir{\'o}, Joaquim and Duong, Luc},
  journal={International Journal of Computer Assisted Radiology and Surgery},
  volume={18},
  number={12},
  pages={2329--2338},
  year={2023}
}


@inproceedings{isola2017image,
  title={Image-to-image translation with conditional adversarial networks},
  author={Isola, Phillip and Zhu, Jun-Yan and Zhou, Tinghui and Efros, Alexei A},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={1125--1134},
  year={2017}
}


@inproceedings{zhou2016learning,
  title={Learning dense correspondence via {3D}-guided cycle consistency},
  author={Zhou, Tinghui and Krahenbuhl, Philipp and Aubry, Mathieu and Huang, Qixing and Efros, Alexei A},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={117--126},
  year={2016}
}


@inproceedings{wang2021instance,
  title={Instance-wise hard negative example generation for contrastive learning in unpaired image-to-image translation},
  author={Wang, Weilun and Zhou, Wengang and Bao, Jianmin and Chen, Dong and Li, Houqiang},
  booktitle={Proceedings of the IEEE/CVF International Conference on Computer Vision (ICCV)},
  pages={14020--14029},
  year={2021}
}


@article{dalmaz2022resvit,
  title={{ResViT}: Residual vision transformers for multimodal medical image synthesis},
  author={Dalmaz, Onat and Yurt, Mahmut and {\c{C}}ukur, Tolga},
  journal={IEEE Transactions on Medical Imaging},
  volume={41},
  number={10},
  pages={2598--2614},
  year={2022}
}


@article{armanious2020medgan,
  title={{MedGAN}: Medical image translation using {GANs}},
  author={Armanious, Karim and others},
  journal={Computerized Medical Imaging and Graphics},
  volume={79},
  pages={101684},
  year={2020}
}


@inproceedings{szegedy2016rethinking,
  title={Rethinking the {Inception} architecture for computer vision},
  author={Szegedy, Christian and Vanhoucke, Vincent and Ioffe, Sergey and Shlens, Jon and Wojna, Zbigniew},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={2818--2826},
  year={2016}
}


@inproceedings{deng2009imagenet,
  title={{ImageNet}: A large-scale hierarchical image database},
  author={Deng, Jia and Dong, Wei and Socher, Richard and Li, Li-Jia and Li, Kai and Fei-Fei, Li},
  booktitle={Proceedings of the IEEE Conference on Computer Vision and Pattern Recognition (CVPR)},
  pages={248--255},
  year={2009}
}


@inproceedings{liu2017unsupervised,
  title={Unsupervised image-to-image translation networks},
  author={Liu, Ming-Yu and Breuel, Thomas and Kautz, Jan},
  booktitle={Proceedings of the Advances in Neural Information Processing Systems (NeurIPS)},
  volume={30},
  year={2017}
}

@article{gretton2012kernel,
  title={A kernel two-sample test},
  author={Gretton, Arthur and Borgwardt, Karsten M and Rasch, Malte J and Sch{\"o}lkopf, Bernhard and Smola, Alexander},
  journal={Journal of Machine Learning Research},
  volume={13},
  number={1},
  pages={723--773},
  year={2012}
}

@article{clement2018immediate,
  title={Immediate hypersensitivity to contrast agents: the French 5-year {CIRTACI} study},
  author={Clement, Olivier and others},
  journal={Lancet Discovery Science},
  volume={1},
  pages={51--61},
  year={2018}
}

@article{fahling2017understanding,
  title={Understanding and preventing contrast-induced acute kidney injury},
  author={F{\"a}hling, Michael and Seeliger, Erdmann and Patzak, Andreas and Persson, Pontus B},
  journal={Nature Reviews Nephrology},
  volume={13},
  number={3},
  pages={169--180},
  year={2017}
}

@article{manoranjan2020a,
  title={Radiological contrast agents and radiopharmaceuticals},
  author={Manoranjan S. D’Souza and Rachel Miguel and Sidhartha D. Ray},
  journal={Side Effects of Drugs Annual},
  volume={42},
  pages={459--471},
  year={2020}
}

@article{wagner2021real,
  title={Real-time respiratory motion compensated roadmaps for hepatic arterial interventions},
  author={Wagner, Martin G and others},
  journal={Medical Physics},
  volume={48},
  number={10},
  pages={5661--5673},
  year={2021}
}

@article{lin2019exploring,
  title={Exploring explicit domain supervision for latent space disentanglement in unpaired image-to-image translation},
  author={Lin, Jianxin and Chen, Zhibo and Xia, Yingce and Liu, Sen and Qin, Tao and Luo, Jiebo},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={43},
  number={4},
  pages={1254--1266},
  year={2019}
}

@article{fan2022tr,
  title={{TR-GAN}: Multi-session future {MRI} prediction with temporal recurrent generative adversarial network},
  author={Fan, Chen-Chen and others},
  journal={IEEE Transactions on Medical Imaging},
  volume={41},
  number={8},
  pages={1925--1937},
  year={2022}
}

@inproceedings{yi2017dualgan,
  title={{DualGAN}: Unsupervised dual learning for image-to-image translation},
  author={Yi, Zili and Zhang, Hao and Tan, Ping and Gong, Minglun},
  booktitle={Proceedings of the IEEE International Conference on Computer Vision (ICCV)},
  pages={2849--2857},
  year={2017}
}

@inproceedings{moriakov2020kernel,
  title={Kernel of {CycleGAN} as a principle homogeneous space},
  author={Moriakov, Nikita and Adler, Jonas and Teuwen, Jonas},
  booktitle={Proceedings of the International Conference on Learning Representations (ICLR)},
  year={2020}
}

@inproceedings{kong2021breaking,
  title={Breaking the dilemma of medical image-to-image translation},
  author={Kong, Lingke and Lian, Chenyu and Huang, Detian and Li, Zhenjiang and Hu, Yanle and Zhou, Qichao},
  booktitle={Proceedings of the Advances in Neural Information Processing Systems (NeurIPS)},
  volume={34},
  pages={1964--1978},
  year={2021}
}

@article{lyu2023generative,
  title={Generative adversarial network--based noncontrast {CT} angiography for aorta and carotid arteries},
  author={Lyu, Jinhao and others},
  journal={Radiology},
  volume={309},
  number={2},
  pages={e230681},
  year={2023}
}

@article{kearney2020attention,
  title={Attention-aware discrimination for {MR}-to-{CT} image translation using cycle-consistent generative adversarial networks},
  author={Kearney, Vasant and others},
  journal={Radiology: Artificial Intelligence},
  volume={2},
  number={2},
  pages={e190027},
  year={2020}
}

@article{tmenova2019cyclegan,
  title={{CycleGAN} for style transfer in {X}-ray angiography},
  author={Tmenova, Oleksandra and Martin, R{\'e}mi and Duong, Luc},
  journal={International Journal of Computer Assisted Radiology and Surgery},
  volume={14},
  pages={1785--1794},
  year={2019}
}

@inproceedings{chen2016infogan,
  title={{InfoGAN}: Interpretable representation learning by information maximizing generative adversarial nets},
  author={Chen, Xi and Duan, Yan and Houthooft, Rein and Schulman, John and Sutskever, Ilya and Abbeel, Pieter},
  booktitle={Proceedings of the Advances in Neural Information Processing Systems (NeurIPS)},
  volume={29},
  year={2016}
}

@inproceedings{higgins2017beta,
  title={{{$\beta$}-VAE}: Learning basic visual concepts with a constrained variational framework},
  author={Higgins, Irina and others},
  booktitle={Proceedings of the International Conference on Learning Representations (ICLR)},
  volume={3},
  year={2017}
}

@article{zhang2023breath,
  title={Breath-hold {CBCT}-guided {CBCT}-to-{CT} synthesis via multimodal unsupervised rrepresentation disentanglement learning},
  author={Zhang, Yiwen and Li, Chuanpu and Dai, Zhenhui and Zhong, Liming and Wang, Xuetao and Yang, Wei},
  journal={IEEE Transactions on Medical Imaging},
  volume={42},
  number={8},
  pages={2313--2324},
  year={2023}
}

@inproceedings{park2020swapping,
  title={Swapping autoencoder for deep image manipulation},
  author={Park, Taesung and others},
  booktitle={Proceedings of the Advances in Neural Information Processing Systems (NeurIPS)},
  volume={33},
  pages={7198--7211},
  year={2020}
}

@inproceedings{chen2022unpaired,
  title={Unpaired deep image dehazing using contrastive disentanglement learning},
  author={Chen, Xiang and others},
  booktitle={Proceedings of the European Conference on Computer Vision (ECCV)},
  pages={632--648},
  year={2022}
}

@article{pizzati2023physics,
  title={Physics-informed guided disentanglement in generative networks},
  author={Pizzati, Fabio and Cerri, Pietro and de Charette, Raoul},
  journal={IEEE Transactions on Pattern Analysis and Machine Intelligence},
  volume={45},
  number={8},
  pages={10300--10316},
  year={2023}
}

@article{qu2024sketch2human,
  title={{Sketch2Human}: Deep Human Generation with Disentangled Geometry and Appearance Constraints},
  author={Qu, Linzi and Shang, Jiaxiang and Ye, Hui and Han, Xiaoguang and Fu, Hongbo},
  journal={IEEE Transactions on Visualization and Computer Graphics},
  year={2024},
  note={{D}OI:{\color{blue}
    \href{http://dx.doi.org/10.1109/TVCG.2024.3403160}{10.1109/TVCG.2024.3403160}}}
}

@article{huang2024spironet,
  title={{SPIRONet}: Spatial-Frequency Learning and Topological Channel Interaction Network for Vessel Segmentation},
  author={Huang, De-Xing and others},
  journal={arXiv:2406.19749},
  year={2024}
}

@inproceedings{ronneberger2015u,
  title={{U-Net}: Convolutional networks for biomedical image segmentation},
  author={Ronneberger, Olaf and Fischer, Philipp and Brox, Thomas},
  booktitle={Proceedings of the International Conference on Medical Image Computing and Computer-Assisted Intervention (MICCAI)},
  pages={234--241},
  year={2015}
}
